Super-Suppression of Long Phonon Mean-Free-Paths in Nano-engineered Si due to Heat Current Anticorrelations

The ability to minimize the thermal conductivity of dielectrics with minimal structural intervention that could affect electrical properties is an important capability for engineering thermoelectric efficiency in low-cost materials such as Si. We recently reported the discovery of special arrangements for nanoscale pores in Si that produce a particularly large reduction in thermal conductivity accompanied by strongly anticorrelated heat current fluctuations, a phenomenon that is missed by the diffuse adiabatic boundary conditions conventionally used in numerical Boltzmann transport models. This manuscript presents the results of molecular dynamics simulations and a Monte Carlo ray tracing model that teases apart this phenomenon to reveal that special pore layouts elastically backscatter long-wavelength heat-carrying phonons. This means that heat carriage by a phonon before scattering is undone by the scattered phonon, resulting in an effective mean-free-path that is significantly shorter than the geometric line-of-sight to the pores. This effect is particularly noticeable for the long-wavelength, long mean-free-path phonons whose transport is impeded drastically more than is expected purely from the usual considerations of scattering defined by the distance between defects. This super-suppression of the mean-free-path below the characteristic length scale of the nanostructuring offers a route for minimizing thermal conductivity with minimal structural impact, while the stronger impact on long wavelengths offers possibilities for the design of band-pass phonon filtering. Moreover, the ray tracing model developed in this paper shows that different forms of correlated scattering imprint a unique signature in the heat current autocorrelation function that could be used as a diagnostic in other nanostructured systems.

==> 4.1.2-MD-results-cross-correlations.tex <==
\subsubsection{Heat Flux Decomposition} \label{sec:Heat_Flux_Decomposition}

If the AC affect is due backscattering of phonons at pores we would expect countervailing heat current fluctuations to be spatially, as well as temporally, correlated. Unfortunately, the  HCACF obtained from MD simulations gives no information on the spatial relationship between thermal fluctuations. To overcome this, we have performed simulations in which we decompose the total instantaneous heat flux into contributions from separate sub-regions in the simulation, and used these to compute the  auto- and cross-correlation of the heat current in different regions. These simulations were performed for Si with and without cylindrical pores and the comparison of the results is shown in Fig.~\ref{fig:cylinder-CCFs} (similar results for other pore geometries are also shown in the SI). The calculations, which are described in detail in Sec.~\ref{sec:computational-methods}, require a few additional steps compared to the calculation of the total HCACF because, unlike the total center of mass, the center of mass of each sub region is not fixed.
    
\begin{figure*}[t]
    \centering
    \includegraphics[width=1\textwidth]{Figures/fig4.jpg}
    \caption{Decomposition of the HCACF. Panel (a) shows the Green-Kubo HCACF for the bulk (gold) and nanoporous (blue) systems. Panels (b) and (c) show the regions used for the spatial decomposition of the heat current in MD simulations of bulk and nanoporous Si, respectively. The matrix of plots in (d) shows the cross-correlations of the heat flux in pairs of regions for the bulk (gold) and nanoporous (blue) systems. The color-coding of the rows and columns matches that of the regions in (b) and (c). The diagonal elements correspond to the regional autocorrelation functions and the remaining figures to the cross-correlation functions. The matrix is symmetric and so the four of the plots in the lower half have been omitted and the space used to show the total HCACF for the two systems.}
    \label{fig:cylinder-CCFs}
\end{figure*}

The regions used for the spatial decomposition in Fig.~\ref{fig:cylinder-CCFs}(c) were chosen carefully, with regions 1--3 located between the two pores in the supercell, and region 4 located to the right of the second pore in the supercell. In the porous Si, regions 1, 3 and 4 are geometrically equivalent. The same regions were used in the simulations of pristine Si, Fig.~\ref{fig:cylinder-CCFs}(b), but in this case all regions are geometrically identical. The matrix of auto- and cross-correlation functions is shown in  Fig.~\ref{fig:cylinder-CCFs}(d), with the region's indicated using the same color coding in the side bar as in Fig.~\ref{fig:cylinder-CCFs}(b\&c) with the 

In bulk Si, all correlation functions between a region with itself (the plots on the diagonal of the matrix) shows two distinct peaks, one at short correlation times corresponding to a heat flux fluctuation with itself, and a much broader and less pronounced peak at a longer correlation interval that comes from phonons that travel through the region and continue around the periodic boundary and back to the region a second time. The heat current cross-correlation functions (HCCCF) between pairs of regions show a time delay before correlation occurs that corresponds to the time of flight for phonons to travel between the regions. For regions that are further away the first peak in correlation becomes broader, reflecting the distribution of $x$ projected velocities of the heat-carrying phonons. 

The HCACF and HCCCF for the Si with cylindrical pores are markedly different from those of the bulk Si. In regions 1, 3 and 4 about the pores, the HCACF decays rapidly to a sharp region of anticorrelation which is dominated by around half of the phonons being backscattered off the immediately adjacent pore. In principle, there could be a second later peak and dip that occurs later due to phonons that are reflected from the more distant pore, but the velocity dispersion or changes in direction of the scattered phonons mean that this is not visible or not present. Region 2 is located right between the pores. It too shows a negative region in the HCACF, but at a later interval, due to the three times longer distance of travel to the pores. That said, the anticorrelation is stronger than for region 1 as it is contributed to by both the left and right traveling phonons. Again, it is notable that there is no secondary positive correlation from phonons that are scattered twice (once at the left and right pores) and then pass through region 2 for the third time. This would be the equivalent to a secondary HCACF dip in the HCACFs in bulk Si. This is significant as it means that phonons are uncorrelated after their second backscattering event.   

The cross-correlations of the nanoporous systems between regions 2 and 1 match the bulk behavior initially, but the initial positive correlation is followed by a long interval of anticorrelation. Importantly, in the nanoporous system, regions 1 and 2 of the HCCCF do not have a secondary peak as seen in the bulk Si which is due to phonons that travel around the periodic boundaries of the system. In the nanoporous Si, the route from region 1 to 2 wrapping around the boundaries requires passing two ranks of pores. In fact, the obstacle that the pores present for phonon scattering is seen most clearly in the HCCCFs between region 4 and regions 1, 2, and 3. In these plots, there is no discernible correlation, either positive or negative.

Together these cross-correlations show definitively that (1) backscattering occurs at pores and not at some other region of the system, (2) that a single row of pores [at least of the size in Fig.~\ref{fig:cylinder-CCFs}(c)] is sufficient to prevent the propagation of heat carriers and (3) that the secondary scattering of phonons is uncorrelated. This resolves an important question from our earlier work where we had simulated the scattering of individual phonon wavepackets colliding with pores~\cite{PhysRevB.102.205405}. The wavepacket simulations revealed that the transmission of phonons past the pores is wavelength dependent, but that when reflection occurs wavepackets scatter back and forth multiple times. This seemed contradictory to the single dip seen in the HCACF. However, the non-equilibrium wavepacket simulations were performed at ultralow temperature, and so lacked a full phonon bath. The decomposed equilibrium MD simulations in Fig.~\ref{fig:cylinder-CCFs} complete the picture, showing that at 300 K the heat-carrying phonons are intrinsically sufficiently long-lived to undergo multiple scattering events, but that they lose (temporal) coherence after a secondary scattering.

